Empirical Analysis of EIP-1559: Transaction Fees, Waiting Time, and Consensus Security

A transaction fee mechanism (TFM) is an essential component of a blockchain protocol. However, a systematic evaluation of the real-world impact of TFMs is still absent. Using rich data from the Ethereum blockchain, the mempool, and exchanges, we study the effect of EIP-1559, one of the earliest-deployed TFMs that depart from the traditional first-price auction paradigm. We conduct a rigorous and comprehensive empirical study to examine its causal effect on blockchain transaction fee dynamics, transaction waiting times, and consensus security. Our results show that EIP-1559 improves the user experience by mitigating intrablock differences in the gas price paid and reducing users' waiting times. However, EIP-1559 has only a small effect on gas fee levels and consensus security. In addition, we find that when Ether's price is more volatile, the waiting time is significantly higher. We also verify that a larger block size increases the presence of siblings. These findings suggest new directions for improving TFMs.

==> Tables/Table4.1.tex <==
\begin{table}[htbp]
    \centering
\begin{tabular}{p{0.2\columnwidth} p{0.2\columnwidth} p{0.2\columnwidth}} 

 \textbf{Period} & \textbf{Start Block} & \textbf{End Block} \\ [0.5ex] 
 \hline
 Pre & 12895000 & 12964999 \\ 
 \hline
 ``During'' & 12965000 & 13034999 \\
 \hline
 Post & 13035000 & 13104999 \\
 \hline
\end{tabular}

\caption{Periods and Block Numbers \kartik{format this like Table 1. It may also be a good idea to instead draw a timeline diagram instead of a table with block numbers and dates and specifying regions as Pre/During/Post} \william{Do you like \cref{fig:timeline}?}}
\label{Table 4.1}
\end{table}


==> Tables/Table5.1.1.tex <==
\begin{table}[!htbp] \centering
\small\setlength{\tabcolsep}{1pt}
\begin{tabular}{@{\extracolsep{5pt}}lccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
& \multicolumn{3}{c}{median gas price} \
\cr \cline{2-4}
\\[-1.8ex] & (1) & (2) & (3) \\
\hline \\[-1.8ex]
$\mathbbm{1}(\text{TxType} == 2)$ & -11.00459$^{***}$ & -11.01356$^{***}$ & -10.83807$^{***}$ \\
  & (0.29886) & (0.29694) & (0.15988) \\
 nblock & 0.00087$^{***}$ & 0.00093$^{***}$ & \\
  & (0.00001) & (0.00001) & \\
EIP-1559 adoption & -4.40374$^{***}$ & 0.12530$^{}$ & \\
  & (0.71369) & (0.71746) & \\
90-block volatility & & 3933.12687$^{***}$ & \\
  & & (99.88466) & \\
 size & & -0.00004$^{***}$ & \\
  & & (0.00000) & \\
 ROI & & -239.97575$^{}$ & \\
  & & (330.82715) & \\
 Intercept & 30.51834$^{***}$ & 5.38495$^{***}$ & 5.24094$^{***}$ \\
  & (0.81693) & (1.08557) & (0.11118) \\
\hline \\[-1.8ex]
 Observations & 133,394 & 133,394 & 133,394 \\
 $R^2$ & 0.18269 & 0.19348 & 0.03330 \\
\hline
\hline \\[-1.8ex]
& \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}

  \begin{tablenotes}
      \footnotesize
      \item Fixed effect regression with median gas price as dependent variable, indicator of transaction type as independent variable, with different sets of controls shown in different columns. Hour fixed effect included in Column (1) and (2), while block fixed effect included in Column (3). Standard errors are in parentheses. Median gas prices were lower for the transactions that adopts EIP-1559 style bidding (type-2) for about 11 Gwei on average. The data frequency is by block.
  \end{tablenotes}
  \caption{Gas Price Paid and Transaction Types}
  %\fanz{1) Luyao to explain how to read the table and interpret the numbers. 2) Double check if $p$ is correct?}}/luyao{The p-value cut-off shall be customized. However, the opportunity cost to revise before submission tomorrow is too high.  Let's leave it for the next revision.}
  \label{Table 5.1.1}
\end{table}
